GlowQ: Group-Shared LOw-Rank Approximation for Quantized LLMs

Quantization techniques such as BitsAndBytes, AWQ, and GPTQ are widely used as a standard method in deploying large language models but often degrades accuracy when using low-bit representations, e.g., 4 bits. Low-rank correction methods (e.g., LQER, QERA, ASER) has been proposed to mitigate this issue, however, they restore all layers and insert error-correction modules into every decoder block, which increases latency and memory overhead. To address this limitation, we propose GlowQ, a group-shared low-rank approximation for quantized LLMs that caches a single shared right factor per input-sharing group and restores only the groups or layers that yield the highest accuracy benefit. GlowQ computes the high-precision projection once per input-sharing group and reuses it across its modules, reducing parameter and memory overhead, and retaining the expressivity of layer-specific corrections. We also propose a selective variant, GlowQ-S, that applies the cached shared module only where it provides the largest benefit. Compared with strong baselines, our approach reduces TTFB by (5.6%) and increases throughput by (9.6%) on average, while reducing perplexity on WikiText-2 by (0.17%) and increasing downstream accuracy by 0.42 percentage points. The selective model GlowQ-S further reduces latency, cutting TTFB by (23.4%) and increasing throughput by (37.4%), while maintaining accuracy within 0.2 percentage points on average. Code is available at https://github.com/ahnselim/GlowQ.

==> tables/with_other_quant.tex <==
\begin{table}
  \centering
  \small
  % 아래 두 줄로 캡션-표 간격 조정 (만약 caption 패키지 쓰면 skip 옵션과 충돌 주의)
  \setlength{\abovecaptionskip}{4pt}
  \setlength{\belowcaptionskip}{4pt}
  % 열 간격 좁히기
  \setlength{\tabcolsep}{3pt}

  \sisetup{table-number-alignment=center, table-text-alignment=center}
  \begin{tabular}{l
                  S[table-format=2.2]
                  S[table-format=2.2]}
    \toprule
    Method      & \text{LLaMA~2-7B} & \text{LLaMA~3.2-3B} \\
    \midrule
    GPTQ                  & 5.64               & 9.32 \\
    {+}GlowQ \textsubscript{\scriptsize(on GPTQ)}    & \textbf{5.60}               & \textbf{8.19} \\
    \cmidrule(lr){1-3}
    BnB       & \bfseries 5.64     & 8.29 \\
    {+}GlowQ \textsubscript{\scriptsize(on BnB)}     & \textbf{5.57}               & \bfseries \textbf{8.10} \\
    \bottomrule
  \end{tabular}
  \label{tab:glowq_ppl}
\end{table}

